Parallel expansion of a fuel pellet plasmoid

The problem of the expansion and assimilation of a cryogenic fuel pellet injected into a hot plasma is considered. Due to the transparency of the plasmoid to ambient particles, it is found that electrons reach a `quasi-equilibrium' (QE) which is characterised by a steady-state on the fastest collisional timescale. The simplified electron kinetic equation of the quasi-equilibrium state is solved. Taking a velocity moment of the electron kinetic equation permits a fluid closure, yielding an evolution equation for the parameters describing the QE distribution function. In contrast to the Braginskii equations, the closure does not require that electrons have a short mean free path compared to the size of density perturbations and permits an anisotropic and highly non-Maxwellian distribution function. Since the QE electron distribution function accounts for both trapped and passing electrons, the self-consistent electric potential that causes the expansion can be properly described, in contrast to earlier models of pellet plasmoid expansion with an unbounded potential. The plasmoid expansion is simulated using both a Vlasov model and a cold fluid model for the ions. During the expansion plasmoid ions and electrons obtain a nearly equal amount of energy; as hot ambient electrons provide this energy in the form of collisional heating of plasmoid electrons, the expansion of a pellet plasmoid is expected to be a potent mechanism for the transfer of energy from electrons to ions on a timescale shorter than that of ion-electron thermalisation.

==> sound-waves.tex <==

\subsection{Ion sound waves}
Ion sound waves are expected to be generated during the plasmoid expansion owing to the perturbations introduced by the time-dependent density and velocity profiles. These sound waves propagate within a highly inhomogenous plasma with spacially-dependent velocity profiles; sound waves will be amplified in some regions and damped in others. The numerical simulations in the previous subsection used spacial grids fine enough to resolve the bulk expansion, but course enough to cause almost complete numerical dissipation of ion sound waves. In this section we derive the dispersion relation for sound waves propagating within the plasmoid and present numerical simulations showing their generation in the extremities of the plasmoid.

We consider the propagation of sound waves in regions where the Boltzmann relation
\begin{equation}
    Zn_i = n_e = \alpha \mathrm{e}^\frac{e\phi}{T_e}
\end{equation}
holds for some electron temperature $T_e$ and constant $\alpha$. This occurs i) within the densest regions of a cold plasmoid, where $T_e = T$, or ii) anywhere within the plasmoid if $T = T_a$ (implying $T_e = T = T_a$). Naturally, outside of the plasmoid, the Boltzmann relation holds with the temperature $T_e = T_a$. From the Boltzmann relation, we obtain the expression
\begin{equation}
    e \frac{\partial \phi}{\partial z} = T_e \frac{\partial \ln n_i}{\partial z}.
\end{equation}

We write $n_i = n_0 + n_1$ and $u_i = u_0 + u_1$ for $(n_0,u_0)$ the `bulk' ion profile of the plasmoid and ambient plasma, and $(n_1,u_1)$ the perturbation to this profile introduced by a sound wave. We introduce the ordering parameter
\begin{equation}
    \omega_S^* = \left|\frac{n_1}{n_0}\right| \ll 1,
\end{equation}
indicating that the density perturbation is small. The velocity perturbation $u_1$ is not necessarily small compared to $u_0$ (which vanishes in the ambient plasma), but we will neglect any nonlinear terms in $u_1$, a standard technique for the analysis of the propagation of sound waves.

Substitution into the cold-ion system \eqref{eq:ion_continuity},\eqref{eq:ion_velocity} (while neglecting nonlinearity in $u_1$) yields the $O\left((\omega_S^*)^0\right)$ equations
\begin{equation}
    \frac{\partial n_0}{\partial t} + \frac{\partial}{\partial z}\left(n_0 u_0\right) = 0,
\end{equation}
\begin{equation}
    \frac{\partial u_0}{\partial t} + u_0 \frac{\partial u_0}{\partial z} + \frac{Z T_e}{m_i}\frac{\partial \ln n_0}{\partial z} = 0,
\end{equation}
which simply describe the evolution of the bulk plasma profile. The $O(\omega_S^*)$ equations, describing the propagation of sound waves, are given by
\begin{equation}
    \frac{\partial n_1}{\partial t} + \frac{\partial}{\partial z}(n_1 u_0 + n_0 u_1) = 0,
\end{equation}
\begin{equation}
    \frac{\partial u_1}{\partial t} + u_1 \frac{\partial u_0}{\partial z} + u_1 \frac{\partial u_0}{\partial z} + \frac{ZT_e}{m_i}\left(\frac{1}{n_0}\frac{\partial n_1}{\partial z} - \frac{n_1}{n_0} \frac{\partial \ln n_0}{\partial z}\right) = 0.
\end{equation}
By substituting
\begin{equation}
    n_1 = a \mathrm{e}^{i(\omega t - kz)},
\end{equation}
\begin{equation}
    u_1 = b \mathrm{e}^{i(\omega t - kz)},
\end{equation}
into the above two equations we obtain the dispersion relation
\begin{equation}
    \omega = u_0 k + i \frac{\partial u_0}{\partial z} \pm \sqrt{\frac{Z T_e}{m_i}}\sqrt{k^2 + \left(\frac{\partial \ln n_0}{\partial z}\right)^2},
\end{equation}
which implies a growth rate
\begin{equation}
    \gamma = - \frac{\partial u_0}{\partial z},
\end{equation}
phase velocity
\begin{equation}
    \frac{\omega}{k} = u_0 \pm \sqrt{\frac{Z T_e}{m_i}}\sqrt{1 + \left(\frac{1}{k}\frac{\partial \ln n_0}{\partial z}\right)^2},
\end{equation}
and group velocity
\begin{equation}
    \frac{\mathrm{d}\omega}{\mathrm{d}k} = u_0 \pm \sqrt{\frac{ZT_e}{m_i}}\frac{k}{\sqrt{k^2 + \left(\frac{\partial \ln n_0}{\partial z}\right)}}.
\end{equation}
The growth rate shows that in regions of plasma decompression ($\partial u_0/\partial z > 0$) sound waves are damped. This is the case within the plasmoid up to the extremities where $n_0 \approx n_a$. In regions of plasma compression ($\partial u_0/\partial z < 0$) sound waves are amplified; this occurs in the extremities of the plasmoid. Therefore we expect weak or nonexistent sound waves inside the plasmoid, but significant generation of sound waves in the extremities. These sound waves will contain energy that would otherwise contribute to bulk ion flow velocity $u_0$ or to the electron thermal energy, so the generation of sound waves `at worst' does not alter the energy balance (their energy being taken entirely from the bulk flow energy), but in reality are likely to obtain at least some of their energy from the electrons. Therefore, the propagation of ion sound waves is likely to act favourably with regards to the electron-ion energy balance (providing yet more energy to the ions at the expense of electrons). Figure \ref{fig:1e23-sound} shows the ion distribution function, density, and flow velocity at $20\,\mathrm{ms}$ for the expansion with the same parameters as Section \ref{sec:expansion_numerical}, showing that waves are generated predominantly in regions of plasma compression.

\begin{figure}
    \centering
    \hspace{0.5cm}
    \includegraphics[width=\textwidth]{1e23-kinetic-collisionless-sound.pdf}
    \caption{Sound waves generated predominantly in the region of plasma compression.}
    \label{fig:1e23-sound}
\end{figure}
